Exposing Limitations of Language Model Agents in Sequential-Task Compositions on the Web

Language model agents (LMA) recently emerged as a promising paradigm on muti-step decision making tasks, often outperforming humans and other reinforcement learning agents. Despite the promise, their performance on real-world applications that often involve combinations of tasks is still underexplored. In this work, we introduce a new benchmark, called CompWoB -- 50 new compositional web automation tasks reflecting more realistic assumptions. We show that while existing prompted LMAs (gpt-3.5-turbo or gpt-4) achieve 94.0% average success rate on base tasks, their performance degrades to 24.9% success rate on compositional tasks. On the other hand, transferred LMAs (finetuned only on base tasks) show less generalization gap, dropping from 85.4% to 54.8%. By balancing data distribution across tasks, we train a new model, HTML-T5++, that surpasses human-level performance (95.2%) on MiniWoB, and achieves the best zero-shot performance on CompWoB (61.5%). While these highlight the promise of small-scale finetuned and transferred models for task compositionality, their performance further degrades under different instruction compositions changing combinational order. In contrast to the recent remarkable success of LMA, our benchmark and detailed analysis emphasize the necessity of building LMAs that are robust and generalizable to task compositionality for real-world deployment.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables_colm/compositional_miniwob.tex <==
\begin{figure*}[t]
\centering
\scalebox{0.8}{
% \includegraphics[width=0.9\linewidth]{figures/compositional_miniwob_230906.pdf}
% \includegraphics[width=0.9\linewidth]{figures/compositional_miniwob_230921.pdf}
\includegraphics[width=\linewidth]{figures/compositional_miniwob_230929.pdf}
}
\vskip -0.1in
\caption{
We design \textit{\compwob{}}, as a novel decision making benchmark for LMAs, by leveraging the high composability of simulated web environments.
We first select base tasks from the original MiniWoB~\citep{shi2017miniwob} based on the brute-force task complexity averaged among existing LMAs. 
% While considering the feasibility, we randomly combine them into a single task (e.g. \texttt{click-option} + \texttt{login-user} $\rightarrow$ \texttt{click-option\_login-user}). The instructions of base tasks are stitched with ``\textbf{and then}''. LMAs are asked to satisfy the given instructions sequentially (e.g. satisfying the success criteria of task \textit{A} $\rightarrow$ \textit{B}).
While considering the feasibility and reality, we systematically combine them into a sequential single task (e.g. \texttt{click-checkboxes-transfer} + \texttt{enter-password} + \texttt{click-dialog}$\rightarrow$ \texttt{click-checkboxes-transfer\_enter-password\_click-dialog}). The instructions of base tasks are stitched with ``\textbf{and then}''. LMAs are asked to satisfy the given instructions sequentially (e.g. satisfying the success criteria of task \textit{A} $\rightarrow$ \textit{B} $\rightarrow$ \textit{C}).
We also implement \textbf{reverse-order instruction} settings, where the instructions are provided upside down (e.g. solve task \textit{B}, and solve task \textit{C}, after solving task \textit{A}). These complex yet controllable strategies make the analysis of LMA's behaviors easy, while maintaining complex and ambiguous aspects of real-world web environments.
}
\vskip -0.2in
\label{fig:compositional_miniwob}
\end{figure*}


==> tables_colm/compwob_performance.tex <==
\begin{tiny}
\begin{landscape}
\begin{table}[ht]
\begin{center}
\scalebox{0.4}{
\begin{tabular}{l|rrrrrrrrrrrrrrrr}
\toprule
\textbf{Task} &\textbf{WebGUM} & \textbf{HTML-T5} & \textbf{HTML-T5++} & \textbf{RCI} (zero) & \textbf{RCI} (first) & \textbf{RCI} (second) & \textbf{RCI} (comb) & \textbf{RCI} (\texttt{gpt-4}) & \textbf{Synapse} (first) & \textbf{Synapse} (second) & \textbf{Synapse} (best) & \textbf{Synapse} (f;\texttt{gpt-4}) & \textbf{Synapse} (s;\texttt{gpt-4}) & \textbf{Synapse} (b;\texttt{gpt-4}) & \textbf{AdaPlanner} & \textbf{AdaPlanner} (\texttt{davinci})\\
\midrule
click-button\_click-checkboxes & 0.210 & 0.700 & 0.790 & 0.370 & 0.710 & 0.730 & 0.800 & 0.880 & 0.810 & 0.840 & 0.840 & 0.980 & 0.840 & 0.980 & 0.060 & 0.890 \\
click-button\_click-checkboxes-transfer & 0.010 & 0.600 & 0.750 & 0.270 & 0.790 & 0.790 & 0.810 & 1.000 & 0.540 & 0.740 & 0.740 & 0.960 & 0.740 & 0.960 & 0.000 & 0.940 \\
click-button\_click-dialog & 0.870 & 0.720 & 0.970 & 0.740 & 0.830 & 0.820 & 0.940 & 1.000 & 1.000 & 0.650 & 1.000 & 1.000 & 0.660 & 1.000 & 0.900 & 0.980 \\
click-button\_click-link & 0.810 & 0.860 & 0.860 & 0.870 & 0.830 & 0.870 & 0.920 & 0.920 & 0.990 & 0.000 & 0.990 & 1.000 & 0.000 & 1.000 & 0.940 & 0.970 \\
click-button\_click-option & 0.600 & 0.840 & 0.840 & 0.580 & 0.650 & 0.370 & 0.710 & 0.420 & 0.920 & 0.870 & 0.920 & 0.960 & 0.880 & 0.960 & 0.000 & 0.860 \\
click-button-sequence\_click-checkboxes & 0.490 & 0.960 & 0.900 & 0.440 & 0.520 & 0.820 & 0.670 & 0.820 & 0.710 & 0.890 & 0.890 & 0.940 & 0.840 & 0.940 & 0.060 & 0.680 \\
click-button-sequence\_click-option & 0.940 & 1.000 & 1.000 & 0.540 & 0.830 & 0.620 & 0.760 & 0.800 & 0.900 & 0.000 & 0.900 & 0.900 & 0.000 & 0.900 & 0.000 & 0.490 \\
click-button-sequence\_login-user-popup & 0.950 & 0.390 & 0.310 & 0.000 & 0.000 & 0.000 & 0.000 & 0.100 & 0.000 & 0.000 & 0.000 & 0.300 & 0.000 & 0.300 & 0.420 & 0.000 \\
click-link\_click-button & 0.900 & 0.980 & 0.970 & 0.790 & 0.830 & 0.970 & 0.980 & 0.980 & 0.010 & 1.000 & 1.000 & 0.000 & 1.000 & 1.000 & 0.950 & 0.800 \\
click-link\_click-dialog & 0.930 & 0.970 & 1.000 & 0.200 & 0.200 & 0.460 & 0.600 & 0.640 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.540 & 0.490 \\
click-link\_click-widget & 0.940 & 0.990 & 0.990 & 0.550 & 0.520 & 0.820 & 0.900 & 0.780 & 0.370 & 0.000 & 0.370 & 0.820 & 0.000 & 0.820 & 0.980 & 0.890 \\
click-link\_enter-text & 0.130 & 0.900 & 1.000 & 0.090 & 0.160 & 0.200 & 0.060 & 0.840 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.860 & 0.920 \\
click-option\_enter-text & 1.000 & 0.970 & 1.000 & 0.380 & 0.130 & 0.410 & 0.500 & 0.880 & 0.000 & 0.000 & 0.000 & 1.000 & 0.000 & 1.000 & 0.770 & 0.960 \\
click-option\_login-user & 0.980 & 1.000 & 0.960 & 0.010 & 0.000 & 0.000 & 0.000 & 0.860 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-option\_navigate-tree & 0.020 & 0.480 & 0.370 & 0.550 & 0.470 & 0.500 & 0.720 & 0.820 & 0.000 & 0.240 & 0.240 & 0.560 & 0.960 & 0.960 & 0.620 & 0.590 \\
click-widget\_enter-password & 0.370 & 0.740 & 0.810 & 0.000 & 0.000 & 0.000 & 0.000 & 0.740 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-widget\_multi-layouts & 0.430 & 0.400 & 0.220 & 0.000 & 0.000 & 0.000 & 0.000 & 0.240 & 0.000 & 0.760 & 0.760 & 0.000 & 1.000 & 1.000 & 0.000 & 0.000 \\
enter-password\_click-option & 1.000 & 0.690 & 0.900 & 0.000 & 0.020 & 0.000 & 0.000 & 0.780 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
login-user\_navigate-tree & 0.000 & 0.040 & 0.140 & 0.020 & 0.010 & 0.000 & 0.000 & 0.700 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
multi-layouts\_login-user & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.100 & 0.720 & 0.000 & 0.720 & 1.000 & 0.000 & 1.000 & 0.010 & 0.000 \\
\midrule
\textbf{Average (two-way)} & \textbf{0.579} & \textbf{0.712} & \textbf{0.739} & \textbf{0.320} & \textbf{0.375} & \textbf{0.419} & \textbf{0.469} & \textbf{0.715} & \textbf{0.349} & \textbf{0.300} & \textbf{0.469} & \textbf{0.521} & \textbf{0.346} & \textbf{0.641} & \textbf{0.356} & \textbf{0.523} \\
\midrule
click-button\_click-option\_login-user & 0.140 & 0.520 & 0.740 & 0.000 & 0.340 & 0.000 & 0.000 & 0.120 & 0.000 & 0.000 & 0.000 & 0.940 & 0.280 & 0.940 & 0.140 & 0.000 \\
click-button-sequence\_click-option\_login-user & 0.300 & 0.200 & 0.770 & 0.520 & 0.740 & 0.680 & 0.840 & 0.560 & 0.720 & 0.000 & 0.720 & 0.660 & 0.000 & 0.660 & 0.000 & 0.000 \\
click-checkboxes\_click-widget\_click-button-sequence & 0.200 & 0.580 & 0.780 & 0.400 & 0.660 & 0.660 & 0.820 & 1.000 & 0.820 & 0.000 & 0.820 & 0.820 & 0.180 & 0.820 & 0.580 & 0.720 \\
click-checkboxes-transfer\_click-button-sequence\_enter-password & 0.000 & 0.010 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.660 & 0.000 & 0.000 & 0.000 & 0.000 & 0.500 & 0.500 & 0.000 & 0.000 \\
click-checkboxes-transfer\_enter-password\_click-dialog & 0.000 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.280 & 0.000 & 0.420 & 0.420 & 0.000 & 0.400 & 0.400 & 0.000 & 0.000 \\
click-dialog\_click-button-sequence\_enter-password & 0.890 & 1.000 & 1.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.700 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-dialog\_click-checkboxes-transfer\_click-widget & 0.140 & 0.690 & 0.560 & 0.140 & 0.540 & 0.340 & 0.400 & 0.680 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-link\_click-button\_click-dialog & 0.730 & 0.940 & 0.980 & 0.240 & 0.270 & 0.480 & 0.610 & 0.600 & 0.000 & 0.600 & 0.600 & 0.000 & 0.620 & 0.620 & 0.560 & 0.580 \\
click-widget\_click-option\_click-dialog & 0.010 & 0.120 & 0.410 & 0.120 & 0.000 & 0.020 & 0.300 & 0.400 & 0.000 & 0.000 & 0.000 & 0.020 & 0.000 & 0.020 & 0.000 & 0.000 \\
enter-password\_click-checkboxes\_login-user-popup & 0.110 & 0.000 & 0.060 & 0.000 & 0.000 & 0.000 & 0.000 & 0.700 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\midrule
\textbf{Average (three-way)} & \textbf{0.252} & \textbf{0.407} & \textbf{0.531} & \textbf{0.142} & \textbf{0.255} & \textbf{0.218} & \textbf{0.297} & \textbf{0.570} & \textbf{0.154} & \textbf{0.102} & \textbf{0.256} & \textbf{0.244} & \textbf{0.198} & \textbf{0.396} & \textbf{0.128} & \textbf{0.130} \\
\midrule
click-button-sequence\_click-widget\_click-link\_click-button\_click-checkboxes\_click-option\_click-dialog & 0.000 & 0.230 & 0.320 & 0.160 & 0.020 & 0.380 & 0.080 & 0.720 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-button-sequence\_click-widget\_click-link\_click-button\_click-checkboxes\_click-option\_click-dialog\_login-user & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.620 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-link\_click-button\_click-checkboxes\_click-dialog & 0.280 & 0.630 & 0.810 & 0.150 & 0.230 & 0.320 & 0.370 & 0.540 & 0.000 & 0.310 & 0.310 & 0.000 & 0.600 & 0.600 & 0.050 & 0.600 \\
click-link\_click-button\_click-checkboxes\_click-option\_click-dialog & 0.180 & 0.430 & 0.780 & 0.200 & 0.180 & 0.370 & 0.360 & 0.560 & 0.000 & 0.060 & 0.060 & 0.000 & 0.620 & 0.620 & 0.020 & 0.490 \\
click-widget\_click-link\_click-button\_click-checkboxes\_click-option\_click-dialog & 0.000 & 0.040 & 0.140 & 0.140 & 0.360 & 0.100 & 0.300 & 0.480 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\midrule
\textbf{Average (n-way)} & \textbf{0.092} & \textbf{0.266} & \textbf{0.410} & \textbf{0.130} & \textbf{0.158} & \textbf{0.234} & \textbf{0.222} & \textbf{0.584} & \textbf{0.000} & \textbf{0.074} & \textbf{0.074} & \textbf{0.000} & \textbf{0.244} & \textbf{0.244} & \textbf{0.014} & \textbf{0.218} \\
\midrule
click-checkboxes-transfer\_multi-layouts\_email-inbox-forward-nl-transition & 0.240 & 0.460 & 0.650 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.220 & 0.440 \\
click-option\_login-user-transition & 0.990 & 1.000 & 0.800 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-option\_multi-layouts\_click-widget\_login-user-popup-transition & 0.190 & 0.220 & 0.130 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
login-user\_navigate-tree-transition & 0.960 & 1.000 & 1.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.460 & 0.000 & 0.000 & 0.000 & 0.340 & 0.000 & 0.340 & 0.000 & 0.000 \\
login-user-popup\_email-inbox-forward-nl-turk-transition & 1.000 & 0.960 & 0.910 & 0.000 & 0.000 & 0.200 & 0.000 & 0.120 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.700 & 0.560 \\
\midrule
\textbf{Average (transition)} & \textbf{0.676} & \textbf{0.728} & \textbf{0.698} & \textbf{0.000} & \textbf{0.000} & \textbf{0.040} & \textbf{0.000} & \textbf{0.116} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.068} & \textbf{0.000} & \textbf{0.068} & \textbf{0.184} & \textbf{0.200} \\
\midrule
click-button\_click-tab-2-hard & 0.240 & 0.550 & 0.510 & 0.080 & 0.120 & 0.260 & 0.340 & 0.580 & 0.280 & 0.040 & 0.280 & 0.960 & 0.320 & 0.960 & 0.260 & 0.280 \\
click-button-sequence\_use-autocomplete & 0.410 & 0.220 & 0.840 & 0.200 & 0.060 & 0.640 & 0.160 & 0.820 & 0.000 & 0.000 & 0.000 & 0.420 & 0.000 & 0.420 & 0.000 & 0.000 \\
click-checkboxes-soft\_enter-password & 0.990 & 0.850 & 0.910 & 0.000 & 0.000 & 0.000 & 0.000 & 0.820 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-checkboxes-soft\_multi-layouts & 0.930 & 0.240 & 0.170 & 0.000 & 0.000 & 0.000 & 0.000 & 0.120 & 0.000 & 0.300 & 0.000 & 0.000 & 0.820 & 0.820 & 0.000 & 0.000 \\
click-dialog\_search-engine & 0.930 & 0.970 & 0.940 & 0.100 & 0.020 & 0.000 & 0.000 & 0.920 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-dialog-2\_click-widget & 0.270 & 0.460 & 0.690 & 0.000 & 0.000 & 0.000 & 0.040 & 0.020 & 0.100 & 0.000 & 0.100 & 0.180 & 0.000 & 0.180 & 0.160 & 0.100 \\
click-dialog-2\_login-user-popup & 0.330 & 0.440 & 0.360 & 0.000 & 0.000 & 0.000 & 0.000 & 0.060 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
click-widget\_click-checkboxes-soft & 0.120 & 0.290 & 0.460 & 0.080 & 0.100 & 0.060 & 0.200 & 0.600 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.100 & 0.140 \\
enter-date\_login-user & 0.990 & 1.000 & 0.230 & 0.000 & 0.020 & 0.000 & 0.060 & 0.500 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.380 & 0.380 \\
use-autocomplete\_click-dialog & 0.000 & 0.000 & 0.000 & 0.000 & 0.080 & 0.000 & 0.080 & 0.060 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\midrule
\textbf{Average (two-way, easy-medium)} & \textbf{0.521} & \textbf{0.502} & \textbf{0.511} & \textbf{0.046} & \textbf{0.040} & \textbf{0.096} & \textbf{0.088} & \textbf{0.450} & \textbf{0.038} & \textbf{0.034} & \textbf{0.038} & \textbf{0.156} & \textbf{0.114} & \textbf{0.238} & \textbf{0.090} & \textbf{0.090} \\
\textbf{Average (total)} & \textbf{0.463} & \textbf{0.566}& \textbf{0.615} & \textbf{0.179} & \textbf{0.225} & \textbf{0.258} & \textbf{0.287} & \textbf{0.560} & \textbf{0.178} & \textbf{0.154} & \textbf{0.254} & \textbf{0.295} & \textbf{0.225} & \textbf{0.414} & \textbf{0.206} & \textbf{0.295} \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{
Per-task success rate on \compwob{}.
}
\label{tab:per_task_compwob_results}
\end{table}
\end{landscape}
\end{tiny}


==> tables_colm/dataset_ratio.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.7}{
\begin{tabular}{l|rrrrrr}
\toprule
% \textbf{Task} & \textbf{Original} (347K) & \textbf{Strat. A} (424K) & \textbf{Strat. B} (361K) & \textbf{Strat. C} (332K) & \textbf{Strat. D} (292K) & \textbf{Strat. E} (259K) \\
\textbf{Task} & \textbf{Original} (347K) & \textbf{Strat. A} (424K) & \textbf{Strat. B} (351K) & \textbf{Strat. C} (322K) & \textbf{Strat. D} (282K) & \textbf{Strat. E} (241K) \\
\midrule
book-flight & 2.88\% & 2.49\% & 2.84\% & 3.11\% & 3.54\% & 4.15\% \\
choose-date &  0.11\% & 1.25\% & 1.42\% & 1.55\% & 1.77\% & 2.07\% \\
choose-date-easy &  0.97\% & 0.84\% & 0.95\% & 1.04\% & 1.19\% & 1.39\% \\
choose-date-medium &  0.64\% & 0.55\% & 0.63\% & 0.69\% & 0.79\% &  0.92\%\\
choose-list & 0.54\% & 1.24\% & 1.42\% & 1.55\% & 1.77\% & 2.07\% \\
click-button & 2.82\% & 2.44\% & 1.39\%& 0.61\%& 1.73\%& 0.81\% \\
click-button-sequence & 2.88\% & 2.49\% & 1.42\%& 0.62\%& 1.77\%& 0.83\% \\
click-checkboxes & 2.81\% & 2.43\% &  1.36\%&  0.55\%&  1.69\%& 0.73\% \\
click-checkboxes-large & 0.57\%  & 2.15\% & 2.46\% &  2.49\%&  3.06\%& 3.58\% \\
click-checkboxes-soft & 2.66\% & 2.30\% & 2.63\% &  2.87\%&  3.27\%& 3.83\% \\
click-checkboxes-transfer & 2.88\% & 2.49\% & 2.85\% &  3.11\%&  1.77\%& 2.07\% \\
click-collapsible  & 1.71\% & 1.48\% & 1.69\% &  1.85\%&  1.06\%& 1.24\% \\
click-collapsible-2 & 0.63\% & 0.55\% & 0.63\% &  0.68\%&  0.78\%&  0.91\% \\
click-color  & 0.74\% & 1.23\% & 1.40\% &  1.53\%&  1.74\%&  2.04\% \\
click-dialog  & 2.88\% & 2.49\% &  2.85\% &  3.11\%&  1.77\%& 0.83\% \\
click-dialog-2  & 0.95\% & 1.36\% & 1.55\% &  1.70\%&  1.93\%&  2.26\% \\
click-link & 2.87\% & 2.48\% & 1.42\% & 0.62\%&  1.76\%&  0.83\% \\
click-menu & 0.93\% & 1.24\% & 1.42\% &  1.55\%&  1.77\%& 2.07\% \\
click-option  & 2.88\% & 2.49\% & 2.84\% & 3.11\%&  1.77\%&  2.07\% \\
click-pie  & 1.07\% & 2.32\% & 2.65\% &  2.90\%&  3.30\%&  3.86\% \\
click-scroll-list & 0.00\% & 1.01\% & 1.16\% &  1.26\%&  1.44\%& 1.69\% \\
click-shades & 0.00\% & 1.25\% &  1.42\%&  1.55\%&  1.77\%&  2.07\% \\
click-shape  & 1.76\% & 1.80\% &  2.05\%&  2.24\%&  2.56\%& 2.99\% \\
click-tab  & 2.88\% & 2.49\% &  2.84\%&  3.10\%& 1.77\%& 2.07\% \\
click-tab-2 & 0.53\% & 0.46\% &  0.52\%&  0.57\%&  0.65\% & 0.76\% \\
click-tab-2-hard  & 0.45\% & 1.67\% & 1.91\%&  2.09\%& 2.38\% & 2.78\% \\
click-test & 2.88\% & 2.49\% & 1.42\%&  0.62\%& 1.77\% & 0.83\% \\
click-test-2  & 2.88\% & 2.49\% &  1.42\%&  0.62\%& 1.77\% & 0.83\% \\
click-widget  & 2.87\% & 2.48\% &  1.41\%&  0.62\%&  1.76\% & 0.82\% \\
count-shape  & 1.69\% & 1.10\% &  1.26\%&  1.37\%&  1.56\% &  1.83\% \\
email-inbox  & 1.49\% & 1.29\% &  1.47\%&  1.60\%&  1.83\% &  2.14\% \\
email-inbox-forward-nl  & 2.88\% & 2.49\% &  2.84\%&  3.11\%&  1.77\% & 2.07\% \\
email-inbox-forward-nl-turk & 1.41\% & 1.22\% &  1.39\%&  1.52\%& 0.86\% & 1.01\% \\
email-inbox-nl-turk  & 1.25\% & 1.08\% &  1.24\%&  1.35\%& 1.54\% & 1.80\% \\
enter-date  & 2.88\% & 2.49\% & 2.85\%&  3.11\%& 3.54\% & 4.15\% \\
enter-password  & 2.88\% & 2.49\% &  2.84\%&  3.10\%& 1.77\% & 2.07\% \\
enter-text  & 2.88\% & 2.49\% &  2.85\%&  3.11\%& 1.77\% & 0.83\% \\
enter-text-dynamic & 2.88\% & 2.49\% & 1.42\%&  0.62\%& 1.77\% & 0.83\% \\
enter-time & 0.00\% & 1.08\% &  1.23\%&  1.35\%& 1.54\% & 1.80\% \\
focus-text & 2.88\% & 2.49\% &  1.42\%&  0.62\%&  1.77\% &  0.83\% \\
focus-text-2  & 2.88\% & 2.49\% &  1.42\%&  0.62\%& 1.77\% & 0.83\% \\
grid-coordinate  & 2.41\% & 2.08\% &  2.38\%&  2.60\%& 1.41\% & 0.55\% \\
guess-number & 0.29\% & 1.25\% &  1.42\%&  1.55\%& 1.77\% & 2.07\% \\
identify-shape & 2.60\% & 2.24\% & 2.56\%&  2.80\%& 1.60\% & 0.75\% \\
login-user & 2.82\% & 2.44\% &  2.79\%&  3.05\%& 1.73\% & 2.03\% \\
login-user-popup  & 2.82\% & 2.44\% &  2.78\%&  3.04\%& 1.73\% & 2.03\% \\
multi-layouts & 2.88\% & 2.49\% &  2.85\%&  3.11\%&  1.77\% & 2.07\% \\
multi-orderings & 2.88\% & 2.49\% &  2.85\%&  3.11\%& 3.54\% & 4.15\% \\
navigate-tree  & 2.84\% & 2.46\% &  2.81\%&  3.07\%& 1.73\% &  2.02\% \\
search-engine  & 2.56\% & 2.21\% &  2.52\%&  2.76\%& 3.14\% & 3.68\% \\
social-media  & 0.76\& & 0.66\% &  0.75\%&  0.82\%& 0.93\% & 1.09\% \\
social-media-all & 0.03\% & 0.02\% &  0.03\%&  0.03\%&  0.03\% & 0.04\% \\
social-media-some & 0.09\& & 0.08\% &  0.09\%&  0.10\%& 0.11\% & 0.13\% \\
tic-tac-toe & 1.14\% & 1.43\% &  1.63\%&  1.78\%&  2.03\% & 2.37\% \\
use-autocomplete & 1.00\% & 0.86\% &  0.99\%&  1.08\%&  1.23\% & 1.44\% \\
use-spinner & 0.15\% & 1.19\% &  1.36\%&  1.48\%& 1.69\% & 1.98\% \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{
Task ratio in rebalanced dataset for HTML-T5++.
}
\label{tab:dataset_ratio_details}
\end{table}


==> tables_colm/error_analysis_compositional_gpt_4.tex <==
\begin{landscape}
\begin{table}[hb]
\begin{center}
% \begin{scriptsize}
\begin{small}
%\begin{sc}
\scalebox{0.75}{
\begin{tabular}{l|l|l|l|l|l}
\toprule
\multicolumn{2}{c|}{\textbf{RCI}~\citep{kim2023rci}} & \multicolumn{2}{c|}{\textbf{AdaPlanner}~\citep{sun2023adaplanner}} & \multicolumn{2}{c}{\textbf{Synapse}~\citep{zheng2023synapse}} \\
\midrule
\multicolumn{2}{l|}{\textit{Click on the link "adipiscing", and then click on the "submit" button}} & \multicolumn{2}{l|}{Click on the link "Augue", and then click on a "button" widget} & \multicolumn{2}{l}{Select 0Qm9EUt, and then enter the username "cristin" and the } \\
\multicolumn{2}{l|}{} & \multicolumn{2}{l|}{} & \multicolumn{2}{l}{password "M5" into the text fields and press login} \\
\midrule
 \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c|}{\textcolor{cb_red}{\XSolidBrush}} & \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c|}{\textcolor{cb_red}{\XSolidBrush}} & \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c}{\textcolor{cb_red}{\XSolidBrush}} \\
1. click //span[text()="adipiscing"]  & 1. click //span[text()="adipiscing"] & \textcolor{cb_green}{1. click //span[text()="Augue"]} & \textcolor{cb_red}{1. click //span[text()="augue"]} & \textcolor{cb_green}{1. click //*[text()="0Qm9EUt"]/input} &  \textcolor{cb_red}{1. click //*[@id="0Qm9EUt"]} \\
\textcolor{cb_green}{2. click //button[text()="submit"]}  & \textcolor{cb_red}{2. click //button[text()="Submit"]} & 2. click //*[@data-type="button"] & 2. click //*[@data-type="button"] & 2. click //*[@id="username"] & 2. click //*[@id="username"] \\
  &  &  &  & 3. type cristin & 3. type cristin \\
  &  &  &  & 4. click //*[@id="password"] & 4. click //*[@id="password"] \\
  &  &  &  & 5. type M5 & 5. type M5 \\
  &  &  &  & 6. click //*[@id="subbtn"] & 6. click //*[@id="subbtn"] \\
  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
% \end{scriptsize}
\end{center}
\vskip -0.1in
\caption{
Failure examples in \compwob{} with advanced models (\texttt{gpt-4}, \texttt{text-davinci-003}).
}
\label{tab:error_gpt4}
\end{table}
\end{landscape}


==> tables_colm/error_analysis_compositional_miniwob.tex <==
\begin{table}[b]
\begin{center}
% \begin{scriptsize}
\begin{small}
%\begin{sc}
\scalebox{0.5}{
\begin{tabular}{l|l|l|l|l|l}
\toprule
\multicolumn{2}{c|}{\textbf{RCI}~\citep{kim2023rci}} & \multicolumn{2}{c|}{\textbf{AdaPlanner}~\citep{sun2023adaplanner}} & \multicolumn{2}{c}{\textbf{Synapse}~\citep{zheng2023synapse}} \\
\midrule
\multicolumn{2}{l|}{\textit{Click button ONE, then click button TWO, and then select whX, 1Nk,}} & \multicolumn{2}{l|}{\textit{Enter the password "UBKR" into both text fields, and then}} & \multicolumn{2}{l}{\textit{Select yE, and then enter "Juan" into the text field and}} \\
\multicolumn{2}{l|}{\textit{fUK3 and click Submit}} & \multicolumn{2}{l|}{\textit{select KwpUv and click Submit}} & \multicolumn{2}{l}{\textit{press Submit}} \\
\midrule
 \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c|}{\textcolor{cb_red}{\XSolidBrush}} & \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c|}{\textcolor{cb_red}{\XSolidBrush}} & \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c}{\textcolor{cb_red}{\XSolidBrush}} \\
\textcolor{cb_green}{1. click //button[@id="subbtn1"]} &\textcolor{cb_red}{1. type //button[@id="subbtn2"]} & \textcolor{cb_green}{1. click //*[@id="password"]} &  & \textcolor{cb_green}{1. click //*[text()="yE"]/input} &  \\
\textcolor{cb_green}{2. click //button[@id="subbtn2"]} &2. click //*[text()="whX"]/input  & 2. type UBKR & 1. type UBKR & 2. click //input[@id="tt"] & 1. click //input[@id="tt"] \\
3. click //*[text()="whX"]/input & 3. click //*[text()="1Nk"]/input & \textcolor{cb_green}{3. click //*[@id="verify"]} &  &  & \textcolor{cb_red}{2. type yE} \\
4. click //*[text()="1Nk"]/input  & 4. click //*[text()="fUK3"]/input & 4. type UBKR & 2. type UBKR & 3. type Juan &  3. type Juan \\
5. click //*[text()="fUK3"]/input  & \textcolor{cb_red}{5. click //*[text()="gSm"]/input} & 5. click //input[@id="ch0"] & 3. click //input[@id="ch0"] & 4. click //*[@id="subbtn"] & 4. click //*[@id="subbtn"] \\
6. click //*[@id="subbtn"] & 6. click //*[@id="subbtn"] & 6. click //*[@id="subbtn"] & 4. click //*[@id="subbtn"] &  &  \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
% \end{scriptsize}
\end{center}
\vskip -0.15in
\caption{
Failure examples in \compwob{}. The left columns have correct plans and the right have failure plans.
LMAs often ignore necessary intermediate steps or predict incorrect action types and XPath.
}
\vskip -0.2in
\label{tab:error_comp_miniwob}
\end{table}

==> tables_colm/error_analysis_compositional_reverse_instruction.tex <==
\begin{table}[b]
\begin{center}
% \begin{scriptsize}
\begin{small}
%\begin{sc}
\scalebox{0.475}{
\begin{tabular}{l|l|l|l|l|l}
\toprule
\multicolumn{2}{c|}{\textbf{RCI}~\citep{kim2023rci}} & \multicolumn{2}{c|}{\textbf{AdaPlanner}~\citep{sun2023adaplanner}} & \multicolumn{2}{c}{\textbf{Synapse}~\citep{zheng2023synapse}} \\
\midrule
\multicolumn{2}{l|}{\textit{Select rJ and click Submit, after clicking on the "yes" button}} & \multicolumn{2}{l|}{\textit{Select OkRi7,  and click Submit, after clicking on the "previous" button}} & \multicolumn{2}{l}{Select 2ld1 and click Submit, after entering the password "Zy4XI"} \\
\multicolumn{2}{l|}{} & \multicolumn{2}{l|}{} & \multicolumn{2}{l}{\textit{into both text fields}} \\
\midrule
 \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c|}{\textcolor{cb_red}{\XSolidBrush}} & \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c|}{\textcolor{cb_red}{\XSolidBrush}} & \multicolumn{1}{c|}{\textcolor{cb_green}{\CheckmarkBold}} & \multicolumn{1}{c}{\textcolor{cb_red}{\XSolidBrush}} \\
\textcolor{cb_green}{1. click //button[text()="yes"]}  & \textcolor{cb_red}{1. click //*[text()="rj"]/input} & 1. click //*[text()="previous"] & 1. click //*[text()="previous"] & \textcolor{cb_green}{1. click //*[@type="password"]} &  \textcolor{cb_red}{1. click //*[text()="2ld1"]/input} \\
\textcolor{cb_green}{2. click //*[text()="rj"]/input} & \textcolor{cb_red}{2. click //button[text()="yes"]} & \textcolor{cb_green}{2. click //*[text()="OkRi7"]/input} & \textcolor{cb_red}{2. type OkRi7} & 2. type Zy4XI & \textcolor{cb_red}{2. click //*[@type="password"][1]} \\
& \textcolor{cb_red}{3. type rj} & 3. click //*[@id="subbtn"] &  3. click //*[@id="subbtn"] & \textcolor{cb_green}{3. click //*[text()="verify"]} & 3. type Zy4XI \\
3. click //*[@id="subbtn"]  & 4. click //*[@id="subbtn"] &  &  & 4. type Zy4XI & \textcolor{cb_red}{4. click //*[@type="password"][2]} \\
  &  &  &  & \textcolor{cb_green}{5. click //*[text()="2ld1"]/input} & 5. type Zy4XI \\
  &  &  &  & 6. click //*[@id="subbtn"] & 6. click //*[@id="subbtn"] \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
% \end{scriptsize}
\end{center}
\vskip -0.15in
\caption{
Failure examples in \compwob{} with \textbf{reverse-order} instructions.
LMAs often fail to parse the instruction into the correct-order plan, and hallucinate unnecessary actions (e.g. \textit{type}). 
}
\vskip -0.2in
\label{tab:error_reverse_instruction}
\end{table}

==> tables_colm/rank_base_tasks.tex <==
\begin{table}[hb]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.69}{
\begin{tabular}{llr}
\toprule
\textbf{Category} & \textbf{Task} & \textbf{Task Difficulty} \\
\midrule
\multirow{26}{*}{\texttt{easy} (0.8 - 1.0)} & click-button & 0.923 \\
 & click-button-sequence & 0.954 \\
 & click-checkboxes & 0.936 \\
 & click-checkboxes-transfer & 0.862 \\
 & click-collapsible & 0.878 \\
 & click-dialog & 0.923 \\
 & click-link & 0.949 \\
 & click-option & 0.839 \\
 & click-tab & 0.898  \\
 & click-test & 1.000 \\
 & click-test-2 & 0.996 \\
 & click-widget & 0.945 \\
 & email-inbox-forward-nl & 0.844 \\
 & email-inbox-forward-nl-turk & 0.804 \\
 & enter-password & 0.896 \\
 & enter-text & 0.922 \\
 & enter-text-dynamic & 0.933 \\
 & focus-text & 0.999 \\
 & focus-text-2 & 0.990 \\
 & grid-coordinate & 0.920 \\
 & identify-shape & 0.918 \\
 & login-user & 0.881 \\
 & login-user-popup & 0.818 \\
 & multi-layouts & 0.832 \\
 & navigate-tree & 0.825 \\
 & unicode-test & 0.900 \\
\midrule
\multirow{23}{*}{\texttt{medium} (0.6 - 0.8)} & choose-date-easy & 0.740 \\
 & click-checkboxes-large & 0.784 \\
 & click-checkboxes-soft & 0.754  \\
 & click-collapsible-2 & 0.693 \\
 & click-color & 0.742 \\
 & click-dialog-2 & 0.780 \\
 & click-menu & 0.607 \\
 & click-pie & 0.769 \\
 & click-shape  & 0.664 \\
 & click-tab-2 & 0.736 \\
 & click-tab-2-hard & 0.651 \\
 & copy-paste & 0.610 \\
 & email-inbox & 0.778 \\
 & email-inbox-nl-turk & 0.779 \\
 & enter-date & 0.714 \\
 & multi-orderings & 0.793 \\
 & read-table & 0.660 \\
 & search-engine & 0.723 \\
 & simple-algebra & 0.799 \\
 & simple-arithmetic & 0.782 \\
 & social-media & 0.733 \\
 & text-transform & 0.737 \\
 & use-autocomplete & 0.782 \\
\midrule
\multirow{16}{*}{\texttt{hard} (0.0 - 0.6)} & book-flight & 0.510 \\
 & choose-date & 0.331 \\
 & choose-date-medium & 0.497 \\
 & choose-list & 0.520 \\
 & click-scroll-list & 0.401 \\
 & click-shades & 0.501 \\
 & copy-paste-2 & 0.547 \\
 & count-shape & 0.536 \\
 & enter-time & 0.521 \\
 & find-word & 0.590 \\
 & guess-number & 0.363 \\
 & social-media-all & 0.432 \\
 & social-media-some & 0.532 \\
 & terminal & 0.592 \\
 & tic-tac-toe & 0.598 \\
 & use-spinner & 0.457 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.2in
\caption{Brute-force task complexity and difficulty classification of MiniWoB. We split 65 tasks into the three category based on the task complexity: \texttt{easy} (0.8 - 1.0), \texttt{medium} (0.6 - 0.8), and \texttt{hard} (0.0 - 0.6).}
\label{tab:miniwob_task_complexity}
\end{table}

==> tables_colm/reverse_performance.tex <==
\begin{tiny}
\begin{landscape}
\begin{table}[ht]
\begin{center}
\scalebox{0.5}{
\begin{tabular}{l|rrrrrrrrrrrr}
\toprule
\textbf{Task} &\textbf{WebGUM} & \textbf{HTML-T5} & \textbf{HTML-T5++} & \textbf{RCI} (zero) & \textbf{RCI} (first) & \textbf{RCI} (second) & \textbf{RCI} (comb) & \textbf{RCI} (\texttt{gpt-4}) & \textbf{Synapse} (first) & \textbf{Synapse} (second) & \textbf{Synapse} (best) & \textbf{AdaPlanner} \\
\midrule
click-button\_click-checkboxes & 0.180 & 0.340 & 0.630 & 0.420 & 0.310 & 0.420 & 0.380 & 0.520 & 0.670 & 0.800 & 0.800 & 0.340\\
click-button\_click-checkboxes-transfer & 0.060 & 0.260 & 0.630 & 0.150 & 0.140 & 0.230 & 0.200 & 0.320 & 0.360 & 0.930 & 0.930 & 0.090\\
click-button\_click-dialog & 0.300 & 0.020 & 0.030 & 0.850 & 0.790 & 0.790 & 0.810 & 0.840 & 0.170 & 0.200 & 0.200 & 0.000\\
click-button\_click-link & 0.010 & 0.050 & 0.040 & 0.430 & 0.500 & 0.430 & 0.460 & 0.560 & 0.870 & 0.000 & 0.870 & 0.970\\
click-button\_click-option & 0.230 & 0.420 & 0.550 & 0.350 & 0.270 & 0.400 & 0.410 & 0.660 & 0.790 & 0.860 & 0.860 & 0.440\\
click-button-sequence\_click-checkboxes & 0.000 & 0.140 & 0.130 & 0.270 & 0.260 & 0.390 & 0.280 & 0.820 & 0.480 & 0.870 & 0.870 & 0.700\\
click-button-sequence\_click-option & 0.000 & 0.020 & 0.110 & 0.360 & 0.420 & 0.320 & 0.490 & 0.920 & 0.350 & 0.000 & 0.350 & 0.550\\
click-button-sequence\_login-user-popup & 0.000 & 0.720 & 0.020 & 0.000 & 0.000 & 0.000 & 0.000 & 0.160 & 0.000 & 0.000 & 0.000 & 0.280\\
click-link\_click-button & 0.910 & 0.750 & 0.580 & 0.840 & 0.760 & 0.800 & 0.830 & 0.920 & 0.000 & 0.670 & 0.670 & 0.950\\
click-link\_click-dialog & 0.450 & 0.050 & 0.230 & 0.330 & 0.430 & 0.470 & 0.880 & 0.660 & 0.000 & 0.000 & 0.000 & 0.200\\
click-link\_click-widget & 0.140 & 0.750 & 0.740 & 0.550 & 0.580 & 0.480 & 0.530 & 0.780 & 0.640 & 0.000 & 0.640 & 0.920\\
click-link\_enter-text & 0.000 & 0.950 & 0.910 & 0.240 & 0.280 & 0.300 & 0.310 & 0.480 & 0.000 & 0.000 & 0.000 & 0.970\\
click-option\_enter-text & 1.000 & 0.660 & 0.750 & 0.570 & 0.650 & 0.650 & 0.640 & 0.800 & 0.000 & 0.000 & 0.000 & 0.590\\
click-option\_login-user & 0.980 & 0.220 & 0.150 & 0.010 & 0.000 & 0.010 & 0.000 & 0.620 & 0.000 & 0.000 & 0.000 & 0.020\\
click-option\_navigate-tree & 0.000 & 0.060 & 0.050 & 0.450 & 0.390 & 0.500 & 0.490 & 0.440 & 0.050 & 0.590 & 0.590 & 0.880\\
click-widget\_enter-password & 0.280 & 0.470 & 0.530 & 0.000 & 0.000 & 0.000 & 0.000 & 0.300 & 0.000 & 0.000 & 0.000 & 0.000\\
click-widget\_multi-layouts & 0.260 & 0.310 & 0.220 & 0.000 & 0.000 & 0.000 & 0.000 & 0.440 & 0.000 & 0.700 & 0.700 & 0.020\\
enter-password\_click-option & 0.960 & 0.160 & 0.900 & 0.000 & 0.000 & 0.000 & 0.000 & 0.920 & 0.000 & 0.000 & 0.000 & 0.000\\
login-user\_navigate-tree & 0.000 & 0.030 & 0.080 & 0.010 & 0.000 & 0.000 & 0.000 & 0.280 & 0.000 & 0.000 & 0.000 & 0.000\\
multi-layouts\_login-user & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.020 & 0.210 & 0.000 & 0.210 & 0.000\\
\midrule
\textbf{Average (two-way)} & \textbf{0.288} & \textbf{0.319} & \textbf{0.364} & \textbf{0.292} & \textbf{0.289} & \textbf{0.310} & \textbf{0.336} & \textbf{0.573} & \textbf{0.230} & \textbf{0.281} & \textbf{0.385} & \textbf{0.396}\\
\midrule
click-button\_click-option\_login-user & 0.250 & 0.140 & 0.220 & 0.020 & 0.000 & 0.000 & 0.000 & 0.200 & 0.000 & 0.000 & 0.000 & 0.220\\
click-button-sequence\_click-option\_login-user & 0.000 & 0.000 & 0.220 & 0.420 & 0.800 & 0.440 & 0.740 & 0.000 & 0.000 & 0.000 & 0.000 & 0.320\\
click-checkboxes\_click-widget\_click-button-sequence & 0.000 & 0.270 & 0.100 & 0.060 & 0.140 & 0.140 & 0.080 & 0.820 & 0.000 & 0.000 & 0.000 & 0.000\\
click-checkboxes-transfer\_click-button-sequence\_enter-password & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.340 & 0.000 & 0.000 & 0.000 & 0.000\\
click-checkboxes-transfer\_enter-password\_click-dialog & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
click-dialog\_click-button-sequence\_enter-password & 1.000 & 0.690 & 0.040 & 0.000 & 0.000 & 0.000 & 0.000 & 0.680 & 0.000 & 0.000 & 0.000 & 0.000\\
click-dialog\_click-checkboxes-transfer\_click-widget & 0.080 & 0.520 & 0.460 & 0.140 & 0.340 & 0.000 & 0.360 & 0.580 & 0.000 & 0.000 & 0.000 & 0.000\\
click-link\_click-button\_click-dialog & 0.040 & 0.050 & 0.130 & 0.180 & 0.320 & 0.320 & 0.310 & 0.360 & 0.000 & 0.000 & 0.000 & 0.000\\
click-widget\_click-option\_click-dialog & 0.000 & 0.000 & 0.000 & 0.120 & 0.220 & 0.160 & 0.140 & 0.120 & 0.000 & 0.000 & 0.000 & 0.000\\
enter-password\_click-checkboxes\_login-user-popup & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.660 & 0.000 & 0.000 & 0.000 & 0.000\\
\midrule
\textbf{Average (three-way)} & \textbf{0.137} & \textbf{0.167} & \textbf{0.117} & \textbf{0.094} & \textbf{0.182} & \textbf{0.106} & \textbf{0.163} & \textbf{0.376} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.054} \\
\midrule
click-button-sequence\_click-widget\_click-link\_click-button\_click-checkboxes\_click-option\_click-dialog & 0.000 & 0.070 & 0.090 & 0.140 & 0.100 & 0.340 & 0.080 & 0.600 & 0.000 & 0.000 & 0.000 & 0.000\\
click-button-sequence\_click-widget\_click-link\_click-button\_click-checkboxes\_click-option\_click-dialog\_login-user & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.180 & 0.000 & 0.000 & 0.000 & 0.000\\
click-link\_click-button\_click-checkboxes\_click-dialog & 0.000 & 0.090 & 0.240 & 0.220 & 0.220 & 0.120 & 0.200 & 0.320 & 0.000 & 0.000 & 0.000 & 0.000\\
click-link\_click-button\_click-checkboxes\_click-option\_click-dialog & 0.000 & 0.060 & 0.260 & 0.170 & 0.120 & 0.140 & 0.170 & 0.380 & 0.000 & 0.000 & 0.000 & 0.000\\
click-widget\_click-link\_click-button\_click-checkboxes\_click-option\_click-dialog & 0.000 & 0.000 & 0.030 & 0.060 & 0.060 & 0.040 & 0.180 & 0.080 & 0.000 & 0.000 & 0.000 & 0.000\\
\midrule
\textbf{Average (n-way)} & \textbf{0.000} & \textbf{0.044} & \textbf{0.124} & \textbf{0.118} & \textbf{0.100} & \textbf{0.128} & \textbf{0.126} & \textbf{0.312} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} \\
\midrule
click-checkboxes-transfer\_multi-layouts\_email-inbox-forward-nl-transition & 0.170 & 0.360 & 0.780 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.140\\
click-option\_login-user-transition & 0.990 & 0.800 & 0.650 & 0.000 & 0.000 & 0.000 & 0.000 & 0.080 & 0.000 & 0.000 & 0.000 & 0.000\\
click-option\_multi-layouts\_click-widget\_login-user-popup-transition & 0.070 & 0.100 & 0.030 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
login-user\_navigate-tree-transition & 1.000 & 1.000 & 0.990 & 0.000 & 0.000 & 0.000 & 0.000 & 0.080 & 0.000 & 0.000 & 0.000 & 0.000\\
login-user-popup\_email-inbox-forward-nl-turk-transition & 0.650 & 0.770 & 0.820 & 0.000 & 0.000 & 0.220 & 0.100 & 0.300 & 0.000 & 0.000 & 0.000 & 0.580\\
\midrule
\textbf{Average (transition)} & \textbf{0.576} & \textbf{0.606} & \textbf{0.654} & \textbf{0.000} & \textbf{0.000} & \textbf{0.044} & \textbf{0.020} & \textbf{0.092} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.144} \\
\midrule
click-button\_click-tab-2-hard & 0.050 & 0.470 & 0.490 & 0.140 & 0.120 & 0.180 & 0.400 & 0.640 & 0.300 & 0.020 & 0.300 & 0.160\\
click-button-sequence\_use-autocomplete & 0.000 & 0.080 & 0.930 & 0.260 & 0.080 & 0.640 & 0.040 & 0.860 & 0.000 & 0.000 & 0.000 & 0.000\\
click-checkboxes-soft\_enter-password & 0.950 & 0.490 & 0.760 & 0.000 & 0.000 & 0.000 & 0.000 & 0.740 & 0.000 & 0.000 & 0.000 & 0.000\\
click-checkboxes-soft\_multi-layouts & 0.940 & 0.390 & 0.260 & 0.000 & 0.000 & 0.000 & 0.000 & 0.200 & 0.000 & 0.420 & 0.000 & 0.000\\
click-dialog\_search-engine & 0.950 & 0.820 & 0.550 & 0.000 & 0.000 & 0.000 & 0.020 & 0.980 & 0.000 & 0.000 & 0.000 & 0.000\\
click-dialog-2\_click-widget & 0.210 & 0.370 & 0.260 & 0.000 & 0.000 & 0.020 & 0.000 & 0.020 & 0.000 & 0.000 & 0.000 & 0.080\\
click-dialog-2\_login-user-popup & 0.380 & 0.360 & 0.330 & 0.000 & 0.000 & 0.000 & 0.000 & 0.020 & 0.000 & 0.000 & 0.000 & 0.000\\
click-widget\_click-checkboxes-soft & 0.090 & 0.240 & 0.290 & 0.080 & 0.080 & 0.120 & 0.080 & 0.520 & 0.000 & 0.000 & 0.000 & 0.000\\
enter-date\_login-user & 0.950 & 0.350 & 0.960 & 0.000 & 0.040 & 0.000 & 0.000 & 0.400 & 0.000 & 0.000 & 0.000 & 0.040\\
use-autocomplete\_click-dialog & 0.000 & 0.000 & 0.000 & 0.000 & 0.080 & 0.000 & 0.000 & 0.120 & 0.000 & 0.000 & 0.000 & 0.000\\
\midrule
\textbf{Average (two-way, easy-medium)} & \textbf{0.452} & \textbf{0.357} & \textbf{0.483} & \textbf{0.048} & \textbf{0.040} & \textbf{0.096} & \textbf{0.054} & \textbf{0.450} & \textbf{0.030} & \textbf{0.044} & \textbf{0.030} & \textbf{0.028}\\
\textbf{Average (total)} & \textbf{0.291} & \textbf{0.297} & \textbf{0.343} & \textbf{0.157} & \textbf{0.170} & \textbf{0.181} & \textbf{0.192} & \textbf{0.435} & \textbf{0.098} & \textbf{0.121} & \textbf{0.160} & \textbf{0.189} \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{
Per-task success rate on \compwob{} with reverse-order instructions.
}
\label{tab:per_task_reverse_results}
\end{table}
\end{landscape}
\end{tiny}


==> tables_colm/summary_table.tex <==
\begin{table}[thb]
\begin{center}
% \begin{scriptsize}
\begin{small}
%\begin{sc}
\scalebox{0.875}{
\begin{tabular}{lcccc}
\toprule
%& \textbf{Base}  & \textbf{Compositional} & \textbf{Reverse-Order} & \textbf{Advanced} \\
%& \textbf{MiniWoB} & \textbf{MiniWoB} & \textbf{Instructions} & \textbf{Models} \\
& Base  &  & Reverse-Order & Advanced \\
& MiniWoB & \compwob{} & Instructions & Models \\
\midrule
%Prompted LMA & \textbf{94.0}\% / \textbf{98.5}\% & 40.9\% / 53.6\% & \textbf{32.0}\% / \textbf{39.1}\% & 58.3\% / 74.6\% \\
%Transferred LMA & 85.4\% / 95.2\% & \textbf{69.6}\% / \textbf{80.1}\% & 30.8\% / 34.5\% & -- \\
Prompted LMA & \textbf{94.0}\% / \textbf{98.5}\% & 24.9\% / 28.7\% & 18.0\% / 19.2\% & 42.3\% / 56.0\% \\
Transferred LMA & 85.4\% / 95.2\% & \textbf{54.8}\% / \textbf{61.5}\% & \textbf{31.0}\% / \textbf{34.3}\% & -- \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
% \end{scriptsize}
\end{center}
\vskip -0.15in
\caption{
Summary of average / max success rate in web automation.
% Prompted LMAs can solve Base MiniWoB better, but suffer from Compositional MiniWoB more than Finetuned LMAs. Finetuned LMAs may not parse the reverse-order instructions correctly.
}
\vskip -0.1in
\label{tab:summary_table}
\end{table}

